Beyond Regularity: Simple versus Optimal Mechanisms, Revisited

A large proportion of the Bayesian mechanism design literature is restricted to the family of regular distributions $\mathbb{F}_{\tt reg}$ [Mye81] or the family of monotone hazard rate (MHR) distributions $\mathbb{F}_{\tt MHR}$ [BMP63], which overshadows this beautiful and well-developed theory. We (re-)introduce two generalizations, the family of quasi-regular distributions $\mathbb{F}_{\tt Q-reg}$ and the family of quasi-MHR distributions $\mathbb{F}_{\tt Q-MHR}$. All four families together form the following hierarchy: $\mathbb{F}_{\tt MHR} \subsetneq (\mathbb{F}_{\tt reg} \cap \mathbb{F}_{\tt Q-MHR}) \subsetneq \mathbb{F}_{\tt Q-reg}$ and $\mathbb{F}_{\tt Q-MHR} \subsetneq (\mathbb{F}_{\tt reg} \cup \mathbb{F}_{\tt Q-MHR}) \subsetneq \mathbb{F}_{\tt Q-reg}$. The significance of our new families is manifold. First, their defining conditions are immediate relaxations of the regularity/MHR conditions (i.e., monotonicity of the virtual value functions and/or the hazard rate functions), which reflect economic intuition. Second, they satisfy natural mathematical properties (about order statistics) that are violated by both original families $\mathbb{F}_{\tt reg}$ and $\mathbb{F}_{\tt MHR}$. Third but foremost, numerous results [BK96, HR09a, CD15, DRY15, HR14, AHN+19, JLTX20, JLQ+19b, FLR19, GHZ19b, JLX23, LM24] established before for regular/MHR distributions now can be generalized, with or even without quantitative losses.

==> source/apx-alpha-regular.tex <==
\section{Comparison with \texorpdfstring{$\alpha$-Strongly Regularity}{Alpha-Strongly Regularity}}
\label{apx:alpha regular discussion}

% \cite{CR14} introduce a parametric distribution family, referred as 

==> source/apx-discussion.tex <==
\section{Further Discussion about Quasi-Regularity/MHR}
\label{apx:further discussion}

==> source/problem.tex <==

\section*{Mechanism Design Set-Up}

In the rest of this work, we consider the problem of {\em prior-independent revenue maximization}.
There are $n \geq 1$ many independent buyers, whose value distributions $v_{i} \sim F_{i}$ for $i \in [n]$ belong to a certain family (known) but otherwise are arbitrary (unknown).
Specifically, we will consider the following four families:
\begin{itemize}
    \item That the $F_{i}$'s are {\em MHR} and can be {\em asymmetric}.
    % \hfill (\Cref{subsec:sample-mhr:asymmetric})
    
    \item That the $F_{i}$'s are {\em MHR} and {\em symmetric} $F_{1} = F_{2} = \dots = F_{n}$.
    % \hfill (\Cref{subsec:sample-mhr:iid})
    
    \item That the $F_{i}$'s are {\em regular} and can be {\em asymmetric}.
    
    \item That the $F_{i}$'s are {\em regular} and {\em symmetric} $F_{1} = F_{2} = \dots = F_{n}$.
\end{itemize}
If other prior information is completely unknown, any nontrivial revenue guarantee is impossible. Rather, for our purpose of prior-independent revenue maximization, we shall access {\em minimal prior information}. Specifically, we will consider the following two kinds of access:
\begin{itemize}
    \item The access is a {\em single sample} of the first order statistic $\sigma \sim F_{(1)}$.

    \yj{this kind of access arguably is ``minimal''. The previous works accesses one sample from every buyer; we use even less prior information.}

    \item The access is a {\em single quantile query} of the first order statistic \red{$\kappa(q) \eqdef F_{(1)}^{-1}(1 - q)$}
    % \yjnote{Is this $(q, F_{(1)}^{-1}(1 - q))$ or $(q, F_{(1)}^{-1}(q))$? We shall follow \cite{ABB23}.}
    for $q \in [0, 1]$.

    \yj{A generalization of \cite{ABB23}.}
\end{itemize}


\begin{definition}[{\sf Sample-Based Uniform Pricing}'s]
{\em scale-invariant} \cite{AB20,HJL20}
\begin{itemize}
    \item a {\sf Deterministic Sample-Based Uniform Pricing} mechanism

    \item a {\sf Randomized Sample-Based Uniform Pricing} mechanism
\end{itemize}
\end{definition}


\begin{definition}[{\sf Query-Based Uniform Pricing}'s]

\end{definition}

benchmarks
\begin{itemize}
    \item {\BayesianMyersonAuction}

    \item {\BayesianUniformPricing}
\end{itemize}


